KnapsackLB: Enabling Performance-Aware Layer-4 Load Balancing

Layer-4 load balancer (LB) is a key building block of online services. In this paper, we empower such LBs to adapt to different and dynamic performance of backend instances (DIPs). Our system, KNAPSACKLB, is generic (can work with variety of LBs), does not require agents on DIPs, LBs or clients, and scales to large numbers of DIPs. KNAPSACKLB uses judicious active probes to learn a mapping from LB weights to the response latency of each DIP, and then applies Integer Linear Programming (ILP) to calculate LB weights that optimize latency, using an iterative method to scale the computation to large numbers of DIPs. Using testbed experiments and simulations, we show that KNAPSACKLB load balances traffic as per the performance and cuts average latency by up to 45% compared to existing designs.

==> back-back-2.tex <==
\section{Background}
\label{sec:back}

%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.37\textwidth, page=1]{figs/back-lb-2.pdf}
\caption{LBs run on multiple instanced called MUXes.}
%%\caption{Options for running L4 LB. Most of the cloud providers use (a); while third-party LBs use (b).}
\vspace{-0.1in}
\label{fig:back:lb}
\end{figure}
%%%%%% end figure %%%%%%%%%%%%%%%%%

%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth, page=1]{figs/back-burst-vm.pdf}
\caption{CPU utilization observed within burstable VM and request-response latency.}
\vspace{-0.1in}
\label{fig:back:burst}
\end{figure}
%%%%%% end figure %%%%%%%%%%%%%%%%%


\if 0
\begin{figure}[t]
\begin{minipage}[b]{0.4\linewidth}
\centering
\includegraphics[width=1\textwidth, page=1]{figs/back-lb.pdf}
\caption{Options for L4 LB. Most of the cloud providers use (a); third-party LBs use (b).}
\label{fig:back:lb}
\end{minipage}
\hspace{0.5cm}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=1\textwidth, page=2]{figs/back-burst-vm.pdf}
\caption{CPU utilization observed within burstable VM and request-response throughput.}
\label{fig:back:burst}
\end{minipage}
\vspace{-0.2in}
\end{figure}
\fi 

An online service deploys multiple servers (called DIPs) to scale and
to provide high availability. The DIPs run behind a load balancer (LB)
that exposes one or more virtual IPs (VIPs) to receive the traffic
from outside the service. In this paper we focus on layer-4 LB that
splits the traffic across DIPs using TCP/IP fields. VIPs offer
multiple benefits for scalability, security and high
availability\cite{ananta:sigcomm13}.

Fig.\ref{fig:back:lb} shows terminologies in using L4 LBs. LB designs run on multiple instances (called MUXes). MUXes intercept the VIP traffic  and split them across DIPs\cite{ananta:sigcomm13, maglev:nsdi16}.

\if 0
Most of the public cloud providers use IP-in-IP encapsulation to route the VIP packets to DIPs\cite{ananta:sigcomm13, maglev:nsdi16}(Fig.\ref{fig:back:lb}(a)). The packets in the reverse direction use Direct Server Return (DSR) bypassing MUXes. Most of the third party designs\cite{haproxy:web, nginx:web} use \textit{proxy} mode (Fig.\ref{fig:back:lb}(b)) where there are TCP connections between clients-MUXes and corresponding connections between MUXes-DIPs. MUXes simply copy traffic between such connections.  
\fi

%% In addition to DSR, public cloud providers also use \textit{Fastpath}\cite{ananta:sigcomm13} to have traffic from clients in the same datacenter go to the DIPs directly -- bypassing MUXes.  

%% Additionally, intra-datacenter traffic also uses fast-path for VIP traffic to go directly to DIPs\cite{ananta:sigcomm13} bypassing MUXes. 

\textbf{DIP selection:} MUXes need to process packets with high throughput and low latency. Thus, they pick DIPs for new \textit{connections} using fast  algorithms such as (weighted) round robin, hash over TCP/IP fields, power of two or (weighted) least connection\cite{lbalgo:web}. However, a long standing assumption for these algorithms to work well is that the \textit{DIPs have same or known capacities} (capacity = max. throughput of a DIP) to process packets so as to not overload DIPs and have good performance across DIPs. Note that the performance depends on the DIP resource utilization (e.g., CPU), which in turn is a function of its capacity and amount of traffic forwarded. There is a growing trend towards DIPs of the same service to have different capacities as detailed in the next section (\S\ref{sec:back:hetero}). Such LB algorithms fall short in providing good performance in such cases (\S\ref{sec:back:limit}).

%% Existing LBs assume that the capacities of the DIPs behind the same VIP are uniform and/or fixed.

\subsection{Different capacity and performance of the DIPs}
\label{sec:back:hetero}

In this section, we describe some of the reasons for DIPs of the same service to have different performance to the same incoming traffic due to: (a) changes in capacity occurring dynamically, (b) mix of DIPs of different types.

\textbf{Change in performance for DIPs due to changes in capacity:} Existing and
recent works have shown that the VMs in cloud have dramatically
different capacities even when they fall in the same VM type (\eg
D3.medium in Azure) (more details in \S\ref{sec:related}). The change
in capacities mainly stems from {\em noisy neighbors,} \ie the
contention from the VMs on the same host. Even if the vCPUs are
isolated, other resources including CPU
caches\cite{contention:euro18}, main memory\cite{contention:micro15,
  contention:hpca13}, and the memory bus are shared. VMs on the same
host contend for such shared resources dynamically, translating to
dynamic DIP capacities. Additionally, our private conversation with a major cloud provider also indicated \textit{dynamic over-subscription}, \ie the number of vCPUs sharing the same physical cores changes dynamically depending on customer demand, resulting in changes in capacities. Importantly, the \textit{changes in capacity are variable and may occur at any time}. Such change in capacities impacts the performance. Imagine that a DIP with a capacity of 100K reqs/sec, and current traffic to the DIP is 70K req/sec. Due to noisy neighbor, the capacity can come down to 60K reqs/sec. If the LB does not react, the incoming traffic to that DIP remains same exceeding the capacity and causing drop in performance (e.g., increase in latency). As we show in the next section, existing LBs do not react well to the dynamic capacities.

\textbf{DIPs with different performance due to VM reassignment:} 
Our private conversation with a major online service owner (using more than 100K VMs) indicated that they don't always use pay-as-you-go model where they dynamically scale up/down VMs based on the demand. The key reason is that public cloud providers don't always have capacity needed, especially during peak hours. As a result, the service owners don't release their VMs. Instead, they reassign it to different parts of their service. Such a reassignment results in DIPs of different types for the same VIP, resulting in DIPs with different performance in the same DIP-pool of a service. 

\textbf{Newer offerings that automatically change performance:} Recent
works such as Harvest VM\cite{harvestvm:osdi20}, Deflatable
VMs\cite{deflation:euro19} or ElasticVM\cite{smartharvest:eurosys21}
call for changing the capacity of VMs dynamically. In fact, AWS and
Azure cloud providers offer \textit{burstable} VMs that are cheaper but whose
capacity changes dynamically\cite{burstaws:web,
  burstazure:web}. Fig.\ref{fig:back:burst} shows the CPU utilization
observed \textit{within} server and the latency for
server-client communication (server runs in burstable VM). Even though
the CPU utilization observed within the VM stays close to 90\% (barring a brief drop to 60\%), the latency for request-response dynamically changes from 4 msec to 50 msec because the hypervisor throttles the CPU starting at time = 8mins. 

\subsection{Limitation of Existing L4 LB}
\label{sec:back:limit}

\if 0
%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth]{figs/back-setup.pdf}
\caption{Setup for evaluating RR and LC policies in HAProxy LB}
\label{fig:back:setup}
\end{figure}
%%%%%% end figure %%%%%%%%%%%%%%%%%

%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth, page=1]{figs/back-limits.pdf}
\caption{Performance of RR in heterogeneous cluster.}
\label{fig:back:limitrr}
\end{figure}
%%%%%% end figure %%%%%%%%%%%%%%%%%

%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth, page=2]{figs/back-limits.pdf}
\caption{Performance of LC in heterogeneous cluster.}
\label{fig:back:limitlc}
\end{figure}
%%%%%% end figure %%%%%%%%%%%%%%%%%
\fi 

%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure*}
\centering
    \begin{minipage}{.3\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figs/back-setup.pdf}
        \vspace{-0.2in}
        \caption{Setup for evaluating RR and LCA policies in HAProxy LB.}
        \label{fig:back:setup}
    \end{minipage}%
    \hspace{0.2cm}
    \begin{minipage}{0.3\textwidth}
        \centering
        %\vspace{-0.35cm}
        \includegraphics[width=1\textwidth, page=1]{figs/back-limits.pdf}
        \vspace{-0.2in}
        %% \vspace{-0.65cm}
        \caption{Performance of RR with changes in capacity.}
        \label{fig:back:limitrr}
    \end{minipage}%
    \hspace{0.2cm}
    \begin{minipage}{0.3\textwidth}
        \centering
        % \vspace{-1.5cm}
        \includegraphics[width=1\textwidth,page=2]{figs/back-limits.pdf}
        \vspace{-0.2in}
        % \vspace{-1cm}
        \caption{Performance of LCA  with changes in capacity.}
        \label{fig:back:limitlc}
    \end{minipage}%
\vspace{-0.1in}
\end{figure*}
%%%%%% end figure %%%%%%%%%%%%%%%%%


We present the shortcomings of existing L4 LBs in adapting to differences in performance. We consider two L4 LBs: (a)
HAProxy\cite{haproxy:web}, a widely used open-sourced LB, and (b)
Microsoft Azure. 

%% We provide a comparison against schemes from the academic literature in \S\ref{sec:related}.

\subsubsection{LBs dont adapt to dynamic changes in DIP performance}
\label{sec:back:limit:dynamic}

We first show that existing LBs dont adapt to dynamic change in DIP performance due to changes in capacity.

\textbf{HAProxy.} Fig.\ref{fig:back:setup} shows our experimental setup. We
have HAProxy running on a 8-core VM. We have three DIPs -- DIP-HC (x2)
and DIP-LC (HC/LC = High/Low Capacity) on 2-core VMs each. All three
DIPs run web server that compute cache intensive task for every HTTP request. DIP-HC VMs have the same
capacity; we change the capacity of DIP-LC by running varying number
of copies of an antagonist process that thrashes caches (and partially consumes CPU). All VMs run in Azure on DS series (non-burstable) CPU running Ubuntu 20.04.

We evaluate all algorithms in HAProxy and present results for 2
popular algorithms -- (a) round-robin (RR), (b) least-connection
(LCA). RR simply rotates new connections across 3 DIPs. LCA uses the
number of active connections as a proxy for load and selects the DIP with the least number of connections when the new connection appears. 

\textbf{Metric of interest:} For both policies, the metric of interest is request-response latency  (for client requests) for all DIPs. We take average for 1 million requests. 

Fig.\ref{fig:back:limitrr} shows the CPU utilization and request-response
latency for RR. We start with all DIPs of same capacity. The X-axis
shows the ratio of capacity of DIP-LC to DIP-HC,  denoted as "Capacity
ratio." When capacity ratio is 100\%, the CPU utilization on all DIPs
is close to 80\%. Next, to emulate the dynamic/different capacity, we
deploy the antagonist process. Note that, the impact of noisy neighbors could be variable and unpredictable. We want to evaluate if RR (and LCA later) can adapt to new capacities automatically without manual intervention from the service owners. However, we found that HAProxy continues to split the traffic in the same way as before. As a result, for lower capacity ratio, as DIP-LC has lower capacity, it hits close to 100\% utilization before DIP-HC VMs. 

%% However, RR fails to exploit the available capacity on DIP-HC. As a result, we found CPU on DIP-HC VMs under-utilized while DIP-LC is fully utilized.

The CPU imbalance also translates in difference in request-response latencies (Fig.\ref{fig:back:limitrr}(b)). Because of dynamic reduction in capacities and HAProxy continuing to send traffic at same rate, DIP-LC sees higher CPU utilization and higher latencies for the same incoming traffic rate. The imbalance in latencies across DIPs only gets worse as capacity ratio decreases. 


\if 0
When capacity ratio is 100\%, the latency on all the three DIPs is roughly same. As we reduce the capacity ratio, because DIP-LC gets fully utilized while DIP-HC VMs are under-utilized, the latency for requests going to DIP-LC increases, while it remains roughly the same for requests going to DIP-HC VMs. HAProxy does not reduce the traffic going to DIP-LC, and ends up with substantial higher latency. 
\fi 

%% This experiment shows that RR policy in HAProxy results in imbalance in CPU utilization (and latency) and cannot load-balance traffic as per capacities. 

Now we turn to LCA and evaluate whether it can balance load as per the
performance. We keep the same setup. Fig.\ref{fig:back:limitlc}(a) and
Fig.\ref{fig:back:limitlc}(b) show the CPU utilization and end-to-end
latency as we decrease the capacity ratio. Surprisingly, despite LCA
being a policy that considers performance, our observations are similar to
RR. As shown in Fig.\ref{fig:back:limitlc}(a), as we decrease the
capacity ratio, there is imbalance in the CPU utilization on DIP-LC compared to DIP-HC VMs. While the imbalance is slightly smaller than RR, it is still prevalent. LCA also results in CPU fully utilized on DIP-LC whereas DIP-HC VMs are under-utilized resulting in higher latencies on DIP-LC compared to DIP-HC VMs.

At first glance, it may seem that LCA will adapt to different performance by assigning more new connections to the DIP with the
fewest connections at that time. A faster DIP will mostly result in fewer connections than the slower counterparts. However, in doing so, it effectively
\textit{splits the number of concurrent connections equally} among
DIPs. DIPs that finish connections faster will get more connections. However, some DIPs (with lower capacity) can get overwhelmed with many concurrent connections. In such cases, LCA never
reduces the concurrent connections on such DIPs. In the previous example with capacity ratio of 60\%, DIP-LC got roughly 27\% of all
connections; all such connections going to DIP-LC overwhelmed DIP-LC and caused higher latency. 

The other algorithms also exhibited CPU and latency imbalance (not shown due to limited space).

%% These experiments show that RR and LCA fall short in balancing the traffic as per the capacities.  

\if 0
\textbf{Why do RR and LCA fail?} RR is simple and fast, but performance agnostic and simply
rotates the new connections across all DIPs. It assigns roughly equal connections to each DIP. However, some DIPs may not have the capacity to handle such connections, while some other DIPs have
more capacity. In such cases, RR will result in different utilization and performance
on different DIPs.
\fi 



\if 0
Imagine a different example with DIP-1 and DIP-2 with
capacities to handle 1 and 8 concurrent requests (due to difference in
cores). To exploit the capacity of DIP-2, LCA will have to assign both DIPs 8 concurrent  requests \textit{overwhelming DIP-1}.
\fi 
%% \ngs{The statement that was here earlier was unclear. Pls clarify if I've oversimplified it.}
%% In the previous experiment, we found that each DIP had 10-12 concurrent connections. 

\begin{table}
\centering 
\caption{Load imbalance using Azure L4 LB.}
\label{tab:back:azurelb}
\begin{tabular}{|c|c|c|}
\hline
DIPs & CPU utilization & Latency\\
\hline
DIP-LC &  84\% & 7.18 msec\\
\hline
DIP-HC & 51\% & 5.00 msec\\
\hline
\end{tabular}
\vspace{-0.1in}
\end{table}

\textbf{Limitations using Azure public L4 LB:} We repeated the above
experiment using Azure L4 LB. We used above 3 DIPs with Azure
LB. Azure LB only provides IP 5-tuple-based load
balancing\cite{azurelb:web}.
%% -- in a way it assumes DIPs of same capacity.
Table \ref{tab:back:azurelb} shows the latency and CPU utilization on
DIP-HC and DIP-LC. Here DIP-LC has 60\% capacity compared to
DIP-HC. Unsurprisingly, as IP 5-tuple-based load balancing is not
inherently capacity and performance aware. We see imbalance in terms of the CPU
utilization as well as latency -- latency of DIP-LC to be
43\% higher than DIP-HC.  


\subsubsection{LBs dont adapt to DIPs with different performance}
\label{sec:back:limit:different}
In the previous section, we showed the different in performance due to dynamic changes in the capacity. In this experiment, we show that LBs dont react to static differences in performance. We have two DIPs behind LB -- one each from DS- and F- series in Azure with same number of cores. Both the DIPs run web server. Again, our metric of interest is request-response latency. We set the weights in proportion to number of cores in HAProxy. We observed F-type VMs to provide 15-20\% lower latency for simple request-response traffic compared to DS-type VMs in Azure. However, both HAProxy and Azure LB \textit{split the traffic equally among such VMs} that did not yield optimal latency. Instead, the latency could be lowered through \textit{un-even split} -- sending more traffic to F-series VM. 

\subsubsection{Changing weights to adapt to capacity} 
As mentioned previously, one of the key limitation of HAProxy and Azure LBs is that they did not automatically adjust the traffic split to adapt to change in performance. However, manual intervention by changing the weights to split the traffic is also not trivial. If some DIPs are suffering from poor performance (hotspots), if too little weight is taken away, that may not clear the hotspots. On other extreme, if too much weight is taken away, it risks hotspots moving somewhere else. \name relieves service operators from deciding weights for optimal performance.

%% These experiments show  existing LBs are unable to respond to differences in performance and result in poor performance on some of the DIPs.


==> back-back.tex <==
\section{Background}
\label{sec:back}

%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.37\textwidth, page=1]{figs/back-lb.pdf}
\caption{Options for running L4 LB. Most of the cloud providers use (a); while third-party LBs use (b).}
\vspace{-0.1in}
\label{fig:back:lb}
\end{figure}
%%%%%% end figure %%%%%%%%%%%%%%%%%

%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth, page=2]{figs/back-burst-vm.pdf}
\caption{CPU utilization observed within burstable VM and request-response throughput.}
\vspace{-0.1in}
\label{fig:back:burst}
\end{figure}
%%%%%% end figure %%%%%%%%%%%%%%%%%


\if 0
\begin{figure}[t]
\begin{minipage}[b]{0.4\linewidth}
\centering
\includegraphics[width=1\textwidth, page=1]{figs/back-lb.pdf}
\caption{Options for L4 LB. Most of the cloud providers use (a); third-party LBs use (b).}
\label{fig:back:lb}
\end{minipage}
\hspace{0.5cm}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=1\textwidth, page=2]{figs/back-burst-vm.pdf}
\caption{CPU utilization observed within burstable VM and request-response throughput.}
\label{fig:back:burst}
\end{minipage}
\vspace{-0.2in}
\end{figure}
\fi 

An online service deploys multiple servers (called DIPs) to scale and
to provide high availability. The DIPs run behind a load balancer (LB)
that exposes one or more virtual IPs (VIPs) to receive the traffic
from outside the service. In this paper we focus on layer-4 LB that
splits the traffic across DIPs using TCP/IP fields. VIPs offer
multiple benefits for scalability, security and high
availability\cite{ananta:sigcomm13}.

Fig.\ref{fig:back:lb} shows terminologies in using L4 LBs. LB designs run on multiple instances (called MUXes). MUXes intercept the VIP traffic from the clients. Most of the public cloud providers use IP-in-IP encapsulation to route the VIP packets to DIPs\cite{ananta:sigcomm13, maglev:nsdi16}(Fig.\ref{fig:back:lb}(a)). The packets in the reverse direction use Direct Server Return (DSR) bypassing MUXes. Most of the third party designs\cite{haproxy:web, nginx:web} use \textit{proxy} mode (Fig.\ref{fig:back:lb}(b)) where there are TCP connections between clients-MUXes and corresponding connections between MUXes-DIPs. MUXes simply copy traffic between such connections.  
 

%% In addition to DSR, public cloud providers also use \textit{Fastpath}\cite{ananta:sigcomm13} to have traffic from clients in the same datacenter go to the DIPs directly -- bypassing MUXes.  

%% Additionally, intra-datacenter traffic also uses fast-path for VIP traffic to go directly to DIPs\cite{ananta:sigcomm13} bypassing MUXes. 

\textbf{DIP selection:} MUXes need to process packets with high throughput and low latency. Thus, they pick DIPs for new \textit{connections} using fast  algorithms such as (weighted) round robin, hash over TCP/IP fields, power of two or (weighted) least connection\cite{lbalgo:web}. However, a long standing assumption for these algorithms to work well is that the \textit{DIP have same or known capacities} (capacity = max. throughput of a DIP) to process packets so as to not overload DIPs and have good performance across DIPs. However, there is a growing trend towards DIPs with different and (importantly) dynamic capacities (\S\ref{sec:back:hetero}) where such algorithms fall short in providing good performance across DIPs (\S\ref{sec:back:limit}).

%% Existing LBs assume that the capacities of the DIPs behind the same VIP are uniform and/or fixed.

\if 0
\textbf{Capacity of the DIPs:} We define capacity of a DIP as the maximum throughput (e.g., requests/sec) provided by the DIP before at least one resource (e.g., CPU) becomes the bottleneck. In the next section, we detail: (a) a growing trend towards DIPs with different and dynamic capacities, (b) limitations of existing LB designs with such DIPs.
\fi 

\subsection{Heterogeneous Capacities of the DIPs}
\label{sec:back:hetero}

\textbf{Dynamic capacities for DIPs in the same VM type:} Existing and
recent works have shown that the VMs in cloud have dramatically
different capacities even when they fall in the same VM type (\eg
D3.medium in Azure) (more details in \S\ref{sec:related}). The change
in capacities mainly stems from {\em noisy neighbors,} \ie the
contention from the VMs on the same host. Even if the vCPUs are
isolated, other resources including CPU
caches\cite{contention:euro18}, main memory\cite{contention:micro15,
  contention:hpca13}, and the memory bus are shared. VMs on the same
host contend for such shared resources dynamically, translating to
dynamic DIP capacities. Our private conversation with a major cloud
provider also indicated \textit{dynamic over-subscription}, \ie the
number of vCPUs sharing the same physical cores changes dynamically
depending on customer demand, resulting in dynamic changes in
capacities.


\if 0
The change in capacities mainly stems from \textit{noisy neighbors}, \ie the contention from the VMs on the same host. Although most of the time, there is isolation between vCPUs of VMs, other resources including CPU caches\cite{contention:euro18}, main memory\cite{contention:micro15, contention:hpca13}, memory bus are shared. Different VMs content for such shared resources dynamically translating in different capacities. Our private conversation with a major cloud provider also indicated \textit{dynamic over-subscription} in terms of physical CPU cores, \ie the number of vCPUs sharing the same physical cores changes dynamically depending on customer demand. Such dynamic over-subscription can also result in changes in capacities. 
\fi 

\textbf{Heterogeneous capacities due to VM reassignment:} Our private conversation with a major online service owner (using more than 100K VMs) indicated that they don't always use pay-as-you-go model where they dynamically scale up/down VMs based on the demand. The key reason is that public cloud providers don't always have capacity needed, especially during peak hours. As a result, the service owners don't release their VMs. Instead, they reassign it to different parts of their service. Such a reassignment again results in DIPs for the same VIP with different capacities. 

%%Lastly, such online services also use DIPs from different generations and SKU resulting in DIPs with different capacities.

\textbf{Newer offerings that automatically change capacity:} Recent
works such as Harvest VM\cite{harvestvm:osdi20}, Deflatable
VMs\cite{deflation:euro19} or ElasticVM\cite{smartharvest:eurosys21}
call for changing the capacity of VMs dynamically. In fact, AWS and
Azure cloud providers offer \textit{burstable} VMs that are cheaper but whose
capacity changes dynamically\cite{burstaws:web,
  burstazure:web}. Fig.\ref{fig:back:burst} shows the CPU utilization
observed \textit{within} server as well as the throughput for
server-client communication (server runs in burstable VM). Even though
the CPU utilization observed within the VM stays close to 90\% (barring a brief drop to 60\%), the throughput dynamically changes from 250 requests/core/sec to just 20 requests/core/sec because the hypervisor throttles the CPU starting at time = 8mins. This also shows that capacity changes dynamically.

\textbf{Different performance across different VM type:} In heterogeneous clusters, different types of VMs may offer different performance. We observed F-type VMs to provide 15-20\% lower latency for simple server-client communication compared to DS-type VMs in Azure. Splitting the traffic equally among such VMs would not yield optimal latency. Instead, the latency could be lowered through \textit{un-even split} -- sending more traffic to F-series VM. 

%% \ngs{in the figure it drops down close to 60\%}

\subsection{Limitation of Existing L4 Load Balancers}
\label{sec:back:limit}

\if 0
%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth]{figs/back-setup.pdf}
\caption{Setup for evaluating RR and LC policies in HAProxy LB}
\label{fig:back:setup}
\end{figure}
%%%%%% end figure %%%%%%%%%%%%%%%%%

%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth, page=1]{figs/back-limits.pdf}
\caption{Performance of RR in heterogeneous cluster.}
\label{fig:back:limitrr}
\end{figure}
%%%%%% end figure %%%%%%%%%%%%%%%%%

%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth, page=2]{figs/back-limits.pdf}
\caption{Performance of LC in heterogeneous cluster.}
\label{fig:back:limitlc}
\end{figure}
%%%%%% end figure %%%%%%%%%%%%%%%%%
\fi 

%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure*}
\centering
    \begin{minipage}{.3\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figs/back-setup.pdf}
        \vspace{-0.2in}
        \caption{Setup for evaluating RR and LCA policies in HAProxy LB.}
        \label{fig:back:setup}
    \end{minipage}%
    \hspace{0.2cm}
    \begin{minipage}{0.3\textwidth}
        \centering
        %\vspace{-0.35cm}
        \includegraphics[width=1\textwidth, page=1]{figs/back-limits.pdf}
        \vspace{-0.2in}
        %% \vspace{-0.65cm}
        \caption{Performance of RR in heterogeneous cluster.}
        \label{fig:back:limitrr}
    \end{minipage}%
    \hspace{0.2cm}
    \begin{minipage}{0.3\textwidth}
        \centering
        % \vspace{-1.5cm}
        \includegraphics[width=1\textwidth,page=2]{figs/back-limits.pdf}
        \vspace{-0.2in}
        % \vspace{-1cm}
        \caption{Performance of LCA in heterogeneous cluster.}
        \label{fig:back:limitlc}
    \end{minipage}%
\vspace{-0.1in}
\end{figure*}
%%%%%% end figure %%%%%%%%%%%%%%%%%


We present the shortcomings of existing L4 LBs in providing good performance when DIPs have
different and dynamic capacities. We consider two L4 LBs: (a)
HAProxy\cite{haproxy:web}, a widely used open-sourced LB, and (b)
Microsoft Azure. 

%% We provide a comparison against schemes from the academic literature in \S\ref{sec:related}.

\textbf{HAProxy.} Fig.\ref{fig:back:setup} shows our experimental setup. We
have HAProxy running on a 8-core VM. We have three DIPs -- DIP-HC (x2)
and DIP-LC (HC/LC = High/Low Capacity) on 2-core VMs each. All three
DIPs run web server on Ubuntu 20.04. DIP-HC VMs have the same
capacity; we change the capacity of DIP-LC by running varying number
of copies of an antagonist process that thrashes caches (and partially consumes CPU). All VMs run in Azure on DS series (non-burstable) CPU.

We evaluate all algorithms in HAProxy and present results for 2
popular algorithms -- (a) round-robin (RR), (b) least-connection
(LCA). RR simply rotates new connections across 3 DIPs. LCA uses the
number of active connections as a proxy for load and selects the DIP with the least number of connections when the new connection appears. For both policies, we measure the CPU utilization and end-to-end latency  (for client requests) for all DIPs, and show average for 1 million requests. 

Fig.\ref{fig:back:limitrr} shows the CPU utilization and end-to-end
latency for RR. We start with all DIPs of same capacity. The X-axis
shows the ratio of capacity of DIP-LC to DIP-HC,  denoted as "Capacity
ratio." When capacity ratio is 100\%, the CPU utilization on all DIPs
is close to 80\%. Next, to emulate the dynamic/different capacity, we
deploy the antagonist process. We don't make any change to HAProxy config as we want to evaluate if RR (and LCA later) can adapt to new capacities. However, we found that as we reduce capacity ratio, the imbalance in the CPU utilization increases. For lower capacity ratio, as DIP-LC has lower capacity, it hits close to 100\% utilization before DIP-HC VMs. However, RR fails to exploit the available capacity on DIP-HC. As a result, we found CPU on DIP-HC VMs under-utilized while DIP-LC is fully utilized.

The CPU imbalance also translates in difference in end-to-end latencies (Fig.\ref{fig:back:limitrr}(b)). When capacity ratio is 100\%, the latency on all the three DIPs is roughly same. As we reduce the capacity ratio, because DIP-LC gets fully utilized while DIP-HC VMs are under-utilized, the latency for requests going to DIP-LC increases, while it remains roughly the same for requests going to DIP-HC VMs. As we decrease the capacity ratio, the latency from DIP-LC only gets worse.

%% This experiment shows that RR policy in HAProxy results in imbalance in CPU utilization (and latency) and cannot load-balance traffic as per capacities. 

Now we turn to LCA and evaluate whether it can balance load as per the
capacities. We keep the same setup. Fig.\ref{fig:back:limitlc}(a) and
Fig.\ref{fig:back:limitlc}(b) show the CPU utilization and end-to-end
latency as we decrease the capacity ratio. Surprisingly, despite LCA
being a policy that considers load, our observations are similar to
RR. As shown in Fig.\ref{fig:back:limitlc}(a), as we decrease the
capacity ratio, there is imbalance in the CPU utilization on DIP-LC compared to DIP-HC VMs. While the imbalance is slightly smaller than RR, it is still prevalent. LCA also results in CPU fully utilized on DIP-LC whereas DIP-HC VMs are under-utilized resulting in higher latencies on DIP-LC compared to DIP-HC VMs.

The other algorithms also exhibited CPU and latency imbalance (not shown due to limited space).

%% These experiments show that RR and LCA fall short in balancing the traffic as per the capacities.  

\textbf{Why do RR and LCA fail?} RR is simple and fast, but performance agnostic and simply
rotates the new connections across all DIPs. It assigns
roughly equal connections to each DIP. However, some DIPs may not have
the capacity to handle such connections, while some other DIPs have
more capacity. In such cases, RR will result in different utilization and performance
on different DIPs.

At first glance, it may seem that LCA will adapt to different
capacities by assigning more new connections to the DIP with the
fewest connections at that time. However, in doing so, it effectively
\textit{splits the number of concurrent connections equally} among
DIPs. DIPs that finish connections faster will get more
connections. However, some DIPs (with lower capacity) can get
overwhelmed with many concurrent connections. In such cases, LCA never
reduces the concurrent connections on such DIPs. In the previous
example with capacity ratio of 60\%, DIP-LC got roughly 27\% of all
connections (in contrast, RR assigned roughly 33\% connections to
DIP-LC). As a result, all such connections going to DIP-LC overwhelmed DIP-LC and observed
higher latency. 

\if 0
Imagine a different example with DIP-1 and DIP-2 with
capacities to handle 1 and 8 concurrent requests (due to difference in
cores). To exploit the capacity of DIP-2, LCA will have to assign both DIPs 8 concurrent  requests \textit{overwhelming DIP-1}.
\fi 
%% \ngs{The statement that was here earlier was unclear. Pls clarify if I've oversimplified it.}
%% In the previous experiment, we found that each DIP had 10-12 concurrent connections. 

\begin{table}
\centering 
\caption{Load imbalance using Azure L4 LB.}
\label{tab:back:azurelb}
\begin{tabular}{|c|c|c|}
\hline
DIPs & CPU utilization & Latency\\
\hline
DIP-LC &  84\% & 7.18 msec\\
\hline
DIP-HC & 51\% & 5.00 msec\\
\hline
\end{tabular}
\vspace{-0.1in}
\end{table}

\textbf{Limitations using Azure public L4 LB:} We repeated the above
experiment using Azure L4 LB. We used above 3 DIPs with Azure
LB. Azure LB only provides IP 5-tuple-based load
balancing\cite{azurelb:web}.
%% -- in a way it assumes DIPs of same capacity.
Table \ref{tab:back:azurelb} shows the latency and CPU utilization on
DIP-HC and DIP-LC. Here DIP-LC has 60\% capacity compared to
DIP-HC. Unsurprisingly, as IP 5-tuple-based load balancing is not
inherently capacity and performance aware. We see imbalance in terms of the CPU
utilization as well as latency -- latency of DIP-LC to be
43\% higher than DIP-HC.  

These experiments show  existing LBs are unable to respond to dynamic DIP capacities and  cause poor performance.


==> back/eval-back.tex <==
\section{Evaluation}
\label{sec:testbed}

\begin{table}
\centering 
\caption{VM details used in evaluation.}
\label{tab:eval:setup}
\small
\begin{tabular}{|c|c|c|c|c|}
\hline
DIPs & DIP-1 to & DIP-17 to & DIP-25 to & DIP-29,30\\
 & DIP-16 & DIP-24 & DIP-28 &\\
\hline
VM type & DS1v2 & DS2v2 & DS3v2 & F8sv2 \\
\hline
\#vCPUs & 1 & 2 & 4 & 8 \\
\hline
\#VMs & 16 & 8 & 4 & 2\\
\hline
\end{tabular}
\vspace{-0.1in}
\end{table}

We evalaute \name using testbed experiments and simulations for large number of DIPs. Our testbed experiments show: (a) \name builds the latency-weight curve fast and requires few points to build the curve, (b) \textit{without any hints} about the capacity, \name is able to compute weights optimally using the ILP to minimize the overall latency, (c) \name  substantially improves the latency compared to round-robin and least-connection based LB. (d) \name handles the dynamics such as failures, capacity changes well, (e) \name can work with other LBs with and without interface to program weights.

\textbf{Setup:} Our setup consists of 41 VMs running in Azure central US datacenter -- there are 30 DIPs with different capacities (summarized in Table \ref{tab:eval:setup}), 1 8-core VM running HAProxy and 8 2-core VMs as clients. Lastly, we have 1 VM each for \name controller and KLM. The DIPs run web server and clients: (a) send the requests to DIPs through HAProxy using multiple processes, (b) measure the end-to-end latency. 

As shown in Table \ref{tab:eval:setup}, we use DIPs of 4 different types. We specifically use VMs across different series (DS and F). The F-series VMs are supposed to be faster than DS-series VMs by up to 2$\times$. However, our measurements found that F-series VM is actually 9\% slower than corresponding DS-series VMs! This also highlights that it is not trivial to calculate the weights just by considering number of cores and clock speed. A system like \name can help automatically calculate and adjust weights based on capacities of the DIPs.

We set the traffic to 70\% of total capacity.

\subsection{Weight assignment in \name}
\label{sec:testbed:curve}

%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure*}
\centering
    \begin{minipage}{.3\textwidth}
        \centering
        \includegraphics[width=1\textwidth, page=1]{figs/eval-weight-hopping.pdf}
        \vspace{-0.2in}
        \caption{Weights used for latency measurements.}
        \label{fig:eval:weights}
    \end{minipage}%
    \hspace{0.2cm}
    \begin{minipage}{0.3\textwidth}
        \centering
        %%\vspace{-0.35cm}
        \includegraphics[width=1\textwidth, page=1]{figs/eval-poly.pdf}
        %% \vspace{-0.65cm}
        \vspace{-0.2in}
        \caption{Curve fitting using polynomial regression.}
        \label{fig:eval:poly}
    \end{minipage}%
    \hspace{0.2cm}
    \begin{minipage}{0.3\textwidth}
        \centering
        % \vspace{-1.5cm}
        \includegraphics[width=1\textwidth,page=2]{figs/eval-weight-hopping.pdf}
        % \vspace{-1cm}
        \vspace{-0.2in}
        \caption{Weights calculated by ILP.}
        \label{fig:eval:ilp}
    \end{minipage}%
\end{figure*}
%%%%%% end figure %%%%%%%%%%%%%%%%%


\textbf{Calculating weights for latency measurements:}
We start our evaluation by calculating the latency-weight curve for all the 30 DIPs. As mentioned in \S\ref{sec:design:curve}, we first start by measuring the latency when weight is 0 and equal (0.033 in this experiment). We then adjust the weights depending on the latency observed as mentioned in algorithm \ref{alg:design:weight}.

Fig.\ref{fig:eval:weights} shows the different weights calculated for 4 different types of DIPs. We randomly chose one DIP from each type (Table \ref{tab:eval:setup}). We make the following observations: (a) the entire experiment to build the weight-latency curve for all DIPs finished in total 10 iterations. Only the DIP-15 took 10 iterations, other DIPs took 9 iterations. Here, we only show the weight calculated by the algorithm \ref{alg:design:weight}, and not by the scheduler (\S\ref{sec:design:schedule}). As a result, the total weight per iteration is not 1. (b) Next, for each iteration, the scheduler scheduled weights in multiple rounds. We observed that scheduler on average took 1.7 rounds for each iteration. Each round was 10 seconds. As a result, the entire experiment finished in less than 3 mins. (c) the weights calculated for measurements vary across DIP types. Also, the $w_{max}$ For the 4 DIPs calculated are 0.04, 0.08, 0.17, 0.33. Recall that the traffic is set to 70\% of total capacity. As a result, even if DIP-15 has 25\% of total capacity, it received $w_{max}$ higher than 25\% (same applies to other DIPs too). One may suggest on doing Weighted Round Robin (WRR) with these weights. We touch upon this in \S\ref{sec:discussion}. 

%% Out of 10 iterations, more than half of the iterations were close to the capacity of the DIPs where we observed high latency and packet drop. 

\textbf{Weight-latency curve using polynomial regression:} Once we measure the latencies for different weights, our next step is to use polynomial regression to fit the curve so that we can estimate the latencies for weights not used in measurements. For polynomial regression, we only use the data for which there was no packet drop. As a result, there are only 4 points for DIP-1 to DIP-14 and 5 points for DIP-15.

Fig.\ref{fig:eval:poly} shows the latency-weight curve for the 4 DIPs of 4 different types. The points show the actual measurements, while the lines show the curve calculated by polynomial regression. It can be seen that the polynomial regression fits the curve well even when it has only a small number of points. 

As we increase the weights, we expect the latency to go up. However, as can be seen in the Fig.\ref{fig:eval:poly}, the latency may not increase monotonically using polynomial regression. To address this limitation, we change the output of the polynomial regression to  increase monotonically by setting the latency for a given weight as maximum of its latency (by regression) and latency at the previous weight (not shown in figure).

\textbf{ILP calculation:} Next, we calculate the weights using ILP described in \S\ref{sec:ilp}. Fig.\ref{fig:eval:ilp} shows the weights calculated to all the 15 DIPs. For DIP-1 to DIP-8, the weights are between 0.026 and 0.029. For DIP-9 to DIP-12, the weights are between 0.057 and 0.061. For DIP-13 and DIP-14, the weights are 0.1 and 0.11. Lastly, the DIP-15 has weight of 0.27. 

ILP assigned more weight to the VM with more capacity (8 core) and comparatively low weight to VMs with low capacity (1 core). ILP assigned weight of 0.27 to DIP-15 even though it has 25\% of total capacity. Similarly, it assigned combined weight of 0.225 to DIP-1 to DIP-8 when these VMs together had 25\% of total capacity. This is because DIP-15 had smaller latency even for higher weight compared  to latencies to DIP-1 to DIP-8 for proportionally smaller weights.

%%the latency is smaller for proportionally smaller weight for VM with larger capacity so ILP assigned higher weight to DIP-15. 


\subsection{Comparing with LC and RR}
\label{sec:eval:rr}

%%%%%%%%%% figure start %%%%%%%%%%%%%%%%
\begin{figure}[t]
\subfigure[CPU utilization]
{
\includegraphics[width = 0.4\textwidth, page=2]{figs/eval-15-node.pdf}
\label{fig:eval:tbcpu}
}
\vspace{-0.1in}
\subfigure[Latency]
{
\includegraphics[width = 0.4\textwidth, page=1]{figs/eval-15-node.pdf}
\label{fig:eval:tblatency}
}
\caption{CPU and latency using 15-node testbed. KLB stands for \name.}
\protect\label{fig:eval:tb}
\vspace{-0.1in}
\end{figure}
%%%%%%%%%%%%%%%%%%%%% figure end %%%%%%%

In this section, we show the improvements in \name compared to Least Connection (LC) -- a policy closest to being capacity aware. We also compare the results against Round Robin (RR) policy. The metrics of interest are end-to-end latency observed by clients and CPU utilization on the DIPs. We show the results for 100K+ requests.  We use two different DIP-pools: (a) same DIP-pool of 15 DIPs as before. (b) smaller DIP-pool of 3 nodes as used in \S\ref{sec:back:limit}. 

%% Let's consider a DIP-pool of 15 DIPs first.
\textbf{15 node DIP-pool:}  Fig.\ref{fig:eval:tbcpu} shows the CPU utilization across all DIP types for RR, LC and \name (KLB). Unsurprisingly, as RR is not capacity aware, it results in high CPU utilization for DIP-1 to  DIP-12 as it assigns higher traffic than the capacity of such DIPs.  Conversely, DIP-13 to DIP-15 show lower CPU utilization as they receive lesser traffic compared to their capacity. LC improves the CPU utilization compared to RR by sending fewer connections to overloaded DIPs but it still results in higher CPU utilization for DIP-1 to DIP-8. In contrast, \name  results in low latency across all DIPs by adjusting the weights as per the capacities. 

Fig.\ref{fig:eval:tblatency} shows the latency across the 4 types of DIPs. In RR, we observe higher latency for DIP-1 to DIP-12 as such DIPs are overloaded. In contrast, latency from DIP-13 to DIP-15 is low as such DIPs are underloaded. LC improves the latency but it still results in high latency due to overloaded DIP-1 to DIP-8. On the other hand, in \name, as the DIPs are not overloaded, we observe low (and uniform) latency across all DIP types. 

This experiment shows that \name improves the latency by up to 80\% for 79\% requests compared to RR, and up to 38\% for 68\% requests compared to LC.

%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth]{figs/testbed-3-nodes.pdf}
\caption{CPU and latency using 3 DIPs of capacity 1$\times$, 0.8$\times$ and 0.6$\times$. KLB denotes \name.}
\label{fig:eval:tb3}
\vspace{-0.1in}
\end{figure}
%%%%%% end figure %%%%%%%%%%%%%%%%%

\textbf{3 node DIP-pool:} In the next experiment, we measure the latency and CPU utilization based on the DIP-pool from \S\ref{sec:back:limit} with capacities closer to each other. In this experiment, we use capacities of 1$\times$, 0.8$\times$ and 0.6$\times$. As shown in Fig.\ref{fig:eval:tb3}, both RR and LC fall short in load balancing the traffic as per capacities, and over-utilize DIP-0.6 (DIP with capacity 0.6$\times$) while there is capacity available on other DIPs. As a result, we also observed higher latency on DIP-0.6. RR and LC sent roughly 33\% and 28.5\% connections to DIP-0.6.

In contrast, \name (denoted by KLB) substantially improves the load balancing. It reduces the CPU utilization on the DIP-0.6 while making use of the available CPU on DIP-1. As a result, we observed similar CPU on all the three nodes. In doing so, \name improved the latency for all the connections that RR and LC sent to DIP-0.6. Compared to RR and LC, \name improved latency by up to 40\% for 37\% and 29\% requests respectively.

\subsection{Handling dynamics}

%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure*}
\centering
    \begin{minipage}{.3\textwidth}
        \centering
        \includegraphics[width=1\textwidth, page=3]{figs/eval-weight-hopping.pdf}
        \vspace{-0.2in}
        \caption{Weight change due to failure of DIP-13.}
        \label{fig:eval:dyn:fail}
    \end{minipage}%
    \hspace{0.2cm}
    \begin{minipage}{0.3\textwidth}
        \centering
        %%\vspace{-0.35cm}
        \includegraphics[width=1\textwidth, page=5]{figs/eval-weight-hopping.pdf}
        \vspace{-0.2in}
        \caption{Weights change due to capacity changes for DIP-13, DIP-14. }
        \label{fig:eval:dyn:cap}
    \end{minipage}%
    \hspace{0.2cm}
    \begin{minipage}{0.3\textwidth}
        \centering
        % \vspace{-1.5cm}
        \includegraphics[width=1\textwidth, page=4]{figs/eval-weight-hopping.pdf}
        % \vspace{-1cm}
        \vspace{-0.2in}
        \caption{Weight change due to traffic change.}
        \label{fig:eval:dyn:traffic}
    \end{minipage}%
\end{figure*}
%%%%%% end figure %%%%%%%%%%%%%%%%%


In this section, we show the change in weights and latency as we address dynamics due to: (a) failures, (b) change in capacity and (c) change in traffic. We use the DIP-pool with 15 DIPs from Table \ref{tab:eval:setup}. We detail our results below:

\textbf{Addressing failures:} In this experiment, we fail DIP-13 while keeping the traffic unchanged. Fig.\ref{fig:eval:dyn:fail} shows the weights before and after the failure. The weight to DIP-13 is 0.106 and 0 before and after the failure. We observed that the weight of the failed DIP \textit{was not} equally split among other DIPs. DIP-1 to DIP-8  saw a cumulative increase of 0.013 in weights. Similarly, DIP-9 to DIP-12 saw cumulative increase of 0.027. Most of the weight of the failed DIP was assigned to DIP-14 and DIP-15 that saw an increase of 0.036 and 0.03 respectively. This was mainly because the VMs with higher capacity (VM-14,15) had more room to absorb traffic with respect to the increase in latency. None of the VMs were overloaded. As the weights were not equally split, it also emphasizes the need for ILP to do more informed decisions.

% Thus, more traffic was assigned to those VMs. 

\textbf{Addressing change in capacity:} In this experiment, we bring back DIP-13 from last experiment but reduce its capacity by 25\% by co-running a process that consumes 1 core. Similarly, we reduce the capacity of DIP-14 by 1 core. We keep total traffic unchanged. This change in capacity was reflected in latency differences for the same weights. As mentioned in \S\ref{sec:dynamics}, we shift the latency-weight curve to left for DIP-13 and DIP-14. Fig.\ref{fig:eval:dyn:cap} again shows the weights before and after the change. Fig.\ref{fig:eval:dyn:cap} shows that \name is able to react to the capacity change and adjust the weights. Interestingly, instead of reducing the weights of DIP-13 and DIP-14 by 25\%, \name reduced the weights assigned to these DIPs by 15-17\%. The remaining weight was mostly assigned to DIP-15 and other DIPs saw a small increase. This is because DIP-15 saw smaller latency increase compared to assigning same weights to DIP-1 to DIP-12.

%% \name assigned most of the weight to DIP-15 as the latency increase was smaller compared to assigning weights to DIP-1 to DIP-12.


%% This is mainly because remaining DIPs didn't have much room to absorb the traffic due to capacity change, and saw disproportionately higher latency increase due to extra traffic. Recall that the latency increases rapidly when the DIPs are close to their capacity. Thus, \name tried to keep the weight (and latency) increase on the other DIPs minimal. Thus, to minimize the overall latency, \name didn't reduce the weight of DIP-13 and DIP-14 by 25\%.  

\textbf{Addressing change in traffic:} In this experiment, we have all the DIPs at their original capacity, and we increase the traffic by 10\%. We detected traffic increase when all DIPs observe increase in latency for the same weights. In such cases, we shift the latency-weight curve to left. Fig.\ref{fig:eval:dyn:traffic} shows the change in weights due to the traffic change. It can be seen that DIP-13, DIP-14 and DIP-15  absorbed most of the extra traffic. This is again because such DIPs have more room to absorb traffic than other DIPs for the same latency increase. In all cases, \name load balanced the traffic as per capacities without overloading any DIP.

These experiments also demonstrate that mechanisms for quick reaction to dynamics are effective. 






==> back/overview-back.tex <==
\section{\name}
\label{sec:overview}

We present \name in this paper. In this section, we sketch \name goals and architecture. \name has following key goals:

\textbf{Generality}: \name intents to work with existing LB designs and empower them to be capacity aware. \name should not require any changes to MUXes, DIPs or clients. As we detail in the next section, \name dynamically changes the \textit{weights} used to split traffic. \name intends to calculate weight calculations and want to free up existing LB (and MUXes) from such calculations.

\textbf{Load balance across DIPs of any capacity!}: Goal of \name is to load balance traffic across DIPs of any capacity. \name should not put any restrictions on the size and capacities of the DIPs.

\textbf{Agent-less and privacy preservation}: \name should not run any agents on the MUXes, DIPs or clients. As such \name does not have access to DIP SKU, CPU utilization or any counters.

\textbf{Everything online}: \name should not require any offline profiling of any component (MUXes, DIPs etc.) and performs all the measurements online.

\subsection{\name overview}
\label{sec:overview:overv}

%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth]{figs/design-cpu-latency.pdf}
\caption{Impact of increasing weights (traffic) on latency and CPU utilization.}
\label{fig:design:weight}
\end{figure}
%%%%%% end figure %%%%%%%%%%%%%%%%%

To meet above goals, we observe that many existing LB designs provide an interface to provide the \textit{weights} for splitting the traffic. On a high level, \name calculates the weights as per the capacities of the DIPs and uses this interface to program the weights. This way, \name can support large number of other LBs. Wherever such an interface is not provided, we use DNS based load balancing as detailed in \S\ref{sec:eval:other}. Secondly, our observation is that applications prefer low end-to-end latency when selecting DIPs at MUXes. Thus, \name calculates the weights so as to minimize the total latency across all DIPs. Additionally, as \name does not have any agents on MUXes or DIPs, it makes all measurements \textit{externally} where it measures  \textit{end-to-end} latency from the DIPs. As shown in Fig.\ref{fig:design:weight}, the latency increases substantially at high CPU utilization against when CPU utilization close to 0. \name selects the weights to optimize total latency across DIPs.

To do so, \name has three key ideas. First, \name decouples the weight calculation from existing LB designs (especially from MUXes) and calculates weights  at a central controller.  It paves way to make decisions optimally while MUXes focus on packet processing with low latency and high throughput. We detail such an architecture in \S\ref{sec:overview:arch}. Second, \name formulates the capacity aware load balancing problem as an Integer Linear Problem (ILP) with a goal to calculate the weights to minimize the total latency across all DIPs of a VIP (we run ILP separately for individual VIPs). The ILP takes \textit{latency at different weights} as an input. We detail the ILP in \S\ref{sec:ilp}. However, running ILP has many challenges detailed in \S\ref{sec:ilp:challenges} -- mainly in getting the latency at multiple weights at scale. \name makes many design choices to address such challenges as detailed in \S\ref{sec:design}.  

\subsection{Architecture}
\label{sec:overview:arch}

%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth]{figs/design-block.pdf}
\caption{\name architecture. Solid and dotted lines denote data traffic and control signals respectively.}
\label{fig:overview:arch}
\end{figure}
%%%%%% end figure %%%%%%%%%%%%%%%%%

%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth]{figs/design-ping-latency.pdf}
\caption{End-to-end (round-trip) latency using different mechanism.}
\label{fig:overview:latency}
\end{figure}
%%%%%% end figure %%%%%%%%%%%%%%%%%


To do so, \name consists of two loosely coupled components: (a) latency measurement, (b) weight calculation as shown in Fig.\ref{fig:overview:arch}. The latency measurement component periodically measures the latency for requests from each DIP. We observed than neither ping (using ICMP) nor TCPping (using SYN/SYNACK) are good indicator if DIPs are reaching capacity as shown in Fig.\ref{fig:overview:latency}. Instead, the latency is measured for application based on the URL provided by the customers/administrators.  Also note that, the request packets do not go through the MUXes. Instead, the requests are sent directly to the DIPs (using IP of a DIP and not VIP) so that we can identify the DIP and also to eliminate the interference of the MUXes. Lastly, we instantiate separate VMs (labelled KLM) in the same VNET as DIPs to measure the latency satisfying the virtual network boundaries. 

The weight calculation component calculates the weights based on the latency measurements. The core of weight calculation algorithm is an ILP based on the weights and corresponding latency for each DIP. It then sends the weights to the LB controller, which then programs the MUXes with the new weighs. The MUXes run the WRR (weighted round robin) using the weights sent by the controller.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\ngs{This section generally seems dispensible to me. Maybe add back
  some of the citations into appropriate categories in the related
  work if you want to be defensive.}

\textbf{Centralized vs. distributed weight calculation:} Alternatively, the MUXes could calculate the weights individually. However, they are limited to run weight calculations due to: (a) fast-path\cite{ananta:sigcomm13} and, (b) MUXes in hardware\cite{duet:sigcomm14, silkroad:sigcomm17, tiara:nsdi22}: that are not extensible to run complex algorithm for weight calculation. In contrast, \name decouples such algorithms from MUXes and runs it at a central controller and thus can work with many hardware/software based MUXes. 

\if 0
\textbf{Centralized vs. distributed weight calculation:} Alternatively, the MUXes could calculate the weights individually. However, there are  challenges: (a) fast-path (\cite{ananta:sigcomm13}): allows clients in datacenters to talk directly to DIPs \textit{bypassing MUXes} reducing packets through MUXes and makes it challenging to enforce weights, (b) MUXes in hardware\cite{duet:sigcomm14, silkroad:sigcomm17, tiara:nsdi22}: may not be extensible to run complex algorithm for weight calculation. In contrast, \name decouples such algorithms from MUXes and runs it at a central controller and thus can work with any hardware/software based MUXes. 
\fi 

%% Software MUXes on the other hand can potentially use the ILP and/or algorithm 1 (\S\ref{sec:design:measure}) when selecting DIPs.

\if 0
\textbf{Supporting layer-7 LBs:} Most of the layer-7 LBs terminate the connections at the L7 LB MUXes\cite{l7lb1:web, l7lb2:web} to perform the load balancing using layer-7 (such as HTTP) fields. As such, L7 MUXes have mechanisms to measure latency and HTTP error codes for DIPs that \name can leverage instead of using its own latency measurements. Other components (to calculate the weights) can be unchanged. 
\fi 

\textbf{Scaling up/down:} We currently haven't focused on scaling up/down the DIP-pool. However, we can alert the admins if the ILP finds at least 1 DIP overloaded. Additionally, using the ILP we can do the \textit{what if analysis} to understand cost, capacity and latency implications of changing DIP-pool. 

%% \textbf{In-band vs. out-of-band measurements:} \name aims for generality and thus made a choice to make latency measurements out-of-band. Recent works\cite{shobhana:hotnets22} focus on load balancing using in-band measurements that (unlike \name) requires access to the MUXes (and dataplane).

%% We leave building such a tool for future work. 

%% \name is agnostic to DIPs types . 
\textbf{Supporting containers and baremetal servers:} \name can easily work with other types of DIPs (e.g., VMs, containers, baremetal servers or a mix) as it only requires IP of the DIPs.

%% and can be easily used with the containers or pods. \name only requires the IP of the backend instances. Once \name has the IPs of the containers or baremetal servers, it will do the load balancing as per their capacities.   

%% \textbf{ILP vs. simpler methods:} One could argue to simply do weighted round robin using $w_{max}$ (calculated in Algorithm 1) obviating a need for ILP. However, such a method does not account for latency. In \name, ILP considers latency and  assigns  weights to minimize total latency.  Lastly, \name can quickly optimize latency during dynamics again due to effective ILP. 

\if 0
\textbf{ILP vs. simpler methods:} One could argue to simply do weighted round robin using $w_{max}$ (calculated in Algorithm 1) obviating a need for ILP. However, such a method does not account for latency. Imagine two DIPs (DIP-1, DIP-2) with DIP-1 having lower latency. Let $w_{max}$ be 0.7 for both DIPs (due to traffic lower than total capacity). Using $w_{max}$, we will end up assigning 0.5 weight to both DIPs. However, ILP considers latency and  assigns more weight to DIP-1 to lower total latency.  Lastly, \name can quickly optimize latency during dynamics again due to effective ILP. 
\fi 

\if 0
\textbf{ILP vs. simpler methods:} As mentioned in \S\ref{sec:testbed:curve}, our algorithm to calculate the latency-weight curve calculates the max. weight for a DIP ($w_{max}$). One could argue to simply use such weights for load balancing obviating a need for ILP. However, note that such a method does not account for latency. Imagine two DIPs (DIP-1, DIP-2) with DIP-1 having lower latency. Let $w_{max}$ be 0.7 for both DIPs (due to traffic lower than total capacity). Using $w_{max}$, we will end up assigning 0.5 weight to both DIPs. However, ILP considers latency and  assigns more weight to DIP-1 to lower total latency.  Lastly, \name can quickly optimize latency during dynamics again due to effective ILP. 
\fi 

%% \textbf{Clustering DIPs with similar latency-weight curve:} such a clustering (e.g., using K-means) can speedup ILP and we leave it for future work.

\textbf{Capacity aware layer-7 LBs:} our learnings can be useful in building capacity aware layer-7 LBs that we leave for the future work. 

%% Also, for setting in \S\ref{sec:testbed:curve}, the ILP calculated the weights with 8\% lower latency compared to when using max. weights.


==> intro-back.tex <==
\section{Introduction}
\label{sec:intro}

A high performance layer-4 load balancer (L4 LB) is one of the key
building blocks of online services. Individual services scale by running on multiple backend servers or VMs with unique IPs (referred as
{\em DIPs}). The service exposes a small number of virtual IPs, termed {\em
  VIPs}, to receive traffic from outside the service. The LB receives traffic coming on the VIPs and distributes
it across DIPs. Recently, there has been significant interest in
improving the scale, availability and cost of the
LB~\cite{ananta:sigcomm13, maglev:nsdi16, duet:sigcomm14,
  silkroad:sigcomm17, beamer:nsdi18, cheetah:nsdi20, tiara:nsdi22, faild:nsdi18}. 

%% Previous work on load balancing assume that capacity of the DIPs is uniform and/or static (\S\ref{sec:related}). 
%% such works have fallen short regarding the fundamental goal of load-balancer, \ie to load-balance the traffic as per the capacities of the DIPs. 
%% However, 
There is a growing trend of DIPs exhibiting different and time-varying
capacities, especially in virtualized clusters. Prior work has shown
that the capacity of VMs with the same type (\eg
D3.medium) may vary up to 40\% due to noisy neighbors: VMs on the
same host compete for shared
resources such as caches and memory buses, resulting in
variation. Additionally, DIPs in the same DIP-pool may be provisioned
with different capacities (\S\ref{sec:back:hetero}). Recent proposals
and new offerings from cloud providers introduce dynamic changes to
the number of virtual CPUs assigned to VMs
(\S\ref{sec:back:hetero}). Together, these factors make
capacities variable across DIPs and over time.

Ideally, LBs should split the traffic to \textit{maximize the performance while conforming to the capacities of DIPs}. However, we find that existing LBs fall short in achieving such a goal in the face of different and dynamic capacities of the DIPs. We consider well-known LBs and
algorithms: (a) HAProxy LB -- one of the widely
used open source LB with all available algorithms, (b) Microsoft Azure
LB. We find that the existing algorithms fall short in splitting traffic as per the capacities, overutilizing some DIPs while underutilizing the rest (\S\ref{sec:back:limit}). Interestingly, the {\em least connections} algorithm, which is specifically built to adapt to variable DIP capacities, also fell short. As a result, the requests going to the over-utilized DIPs suffered poor performance (2$\times$ higher
latency than other DIPs). Lastly, we note that many existing LBs often remove DIPs suffering from poor performance, instead of
adapting to their performance.

\if 0
In this paper, we revisit the first order question on how L4 LBs split traffic. We argue that LBs
should \textit{pack} load according to the dynamic capacities of DIPs, making
it possible to pack higher load onto DIPs with higher capacities.  However, the key challenge is determining how much load is safe to direct to or away from a DIP without adversely impacting service performance.
\fi 

In this paper, we revisit the first order question on how L4 LBs split traffic. We argue that L4 LB problem should be modeled as a \textit{Knapsack problem}\cite{knapsack:book} to pack the load as per the capacities of the DIPs to optimize service performance. The key challenge is determining how much load is safe to direct to or away from a DIP without adversely impacting service performance.

\if 0
should \textit{pack} load according to the dynamic capacities of DIPs, making
it possible to pack higher load onto DIPs with higher capacities.  However, the key challenge is determining how much load is safe to direct to or away from a DIP without adversely impacting service performance.
\fi 

This paper presents \name, a ``meta'' LB design that enables other LBs
to become performance-aware. \name does
not intent to add to the impressive list of existing LB designs. Instead, \name
enables setting the DIP weights for any LB that can implement
weighted load balancing. A significant number of LB systems provide an
interface to specify the weights, including AVI\cite{avi:web},
Nginx\cite{nginx:web}, Duet\cite{duet:sigcomm14}, and
HAProxy\cite{haproxy:web}. \name frees admins from configuring weights
according to DIP performance that are either static or dynamic. In
doing so, it leverages the availability and scalability of existing LB
designs while endowing them with performance awareness.

%%\name works with unmodified DIPs, LBs, and clients (\S\ref{sec:overview}). 

At a high level, using SDN principles, \name decouples weight computation from LBs and does it at a central controller. This enables \name to make optimal decisions with a \textit{global view} across DIPs. In \name, we use request-response latency as a proxy for the performance. \name uses active probing
judiciously to learn a {\em per-DIP weight-latency curve}: a mapping
from a weight to the DIP's average response latency, should
that weight be applied to that DIP. This mapping is used to drive an
Integer Linear Program (ILP) that computes LB weights to pack load
into DIPs, while minimizing the average response latency
across DIPs. The \name\ controller uses the LB's existing
interface to configure DIP weights. In doing so, \name does not require any changes to DIPs, clients, or the LB data plane.

\if 0
\name also adds new client VMs inside
the service's virtual network to perform active measurements. We show
that these additional VMs incur a miniscule cost in exchange for
\name's benefits (\S\ref{sec:testbed}).
\fi 

%% with many of the
%% measurements becoming stale before the probing %% completes


\name addresses three key technical challenges to achieve its goals
(\S\ref{sec:overview:key}). First, issuing probes naively for the
set of all possible weights would require an impractically high number
of latency measurements across hundreds of DIPs. \name
implements just a few measurements (\S\ref{sec:design:curve},
\S\ref{sec:design:measure}), each adapting from the results of the
past measurements, and runs curve-fitting to learn a weight-latency
curve that works well across a wide range of weights.

Second, running an ILP that handles hundreds of DIPs with fine-grained
DIP weight settings is computationally expensive. \name uses a
multi-step ILP to substantially speed up the calculation of DIP
weights. Specifically, in each step, \name runs an ILP that
progressively zooms into finer-grained weight settings per DIP,
instead of calculating weights in one shot
(\S\ref{sec:design:runtime}).

Third, a weight-latency mapping learned at some fixed load
arriving at an LB could become stale. Specifically, the
load placed on a DIP, and hence its response latency, depends
on both the LB's aggregate incoming load and the DIP's
weight. \name avoids learning a new weight-latency curve for each
aggregate load. Instead, \name adapts quickly to variations in traffic
rate by rescaling and shifting its learned weight-latency curve
(\S\ref{sec:dynamics}).

\if 0
\name is based on three key ideas. First, inspired by SDN principles, it decouples the weight calculation from individual LB instances, and calculates the weights at a central controller. The benefits are twofold: (a) it frees up LB dataplane from weight calculation and helps it to be high performant and provide low latency, high throughput packet processing, (b) it helps implement more informed designs for weight calculation at the central controller. 

%% \name uses an ILP (detailed below) at the controller to calculate weights using end-to-end latency between requests and responses.

%% We observe that when traffic reaches the capacity of the DIPs, it results in increased end-to-end latency and packet drops due to queuing delays and contention. Thus, by monitoring the latency and drop, we gauge if traffic is reaching the capacity of the DIPs. 

Second, as a part of load packing, we formulate an Integer Linear Program (ILP) to calculate the LB weights to minimize the total end-to-end latency across DIPs of a VIP as applications value better latencies. While an ILP based packing is appealing, it is also challenging. As detailed in \S\ref{sec:ilp}, the ILP takes the mapping between weights and latency as an input. However, building such a mapping at scale with 100s of latency measurements for each DIP is not trivial. Additionally, again at scale, the ILP becomes computationally expensive.

Our third key idea is to speed up building the mapping between weights and latency for individual DIPs. We observed that we can make-do with latency measurement at small number of weights and use curve-fitting. Next, we use an idea inspired by TCP congestion control to hop different weights to reduce number of latency measurements and get rough estimate of capacity of DIPs. Lastly, we use multi-step ILP to substantially speed up weight calculation. 

\fi

%% To the best of our knowledge, \name is a novel approach to build
%% capacity aware L4 LBs.
We evaluate a 41-VM prototype implementation of \name (\S\ref{sec:impl}) on an Azure public cloud 
and also at larger scale using simulations. Our results (\S\ref{sec:testbed}) show: (a) \name can
adjust the weights as per the capacities of the DIPs. (b) In doing so,
it cuts the latency up to 45\% for up to 79\% requests. (c) \name
adapts to changes in the cluster in terms of capacity, traffic,
and failures. (d) \name solves ILP quickly using optimizations. (e) \name can work with wide range of other LBs. (f) \name incurs only a
small overhead in terms of cores and costs.

This work does not raise any ethical issues.

\if 0
In summary, we make the following contributions: (a) we show that existing LB algorithms (especially least connection algorithm tailored for handling different capacities) fall short in load balancing traffic as per capacities of the DIPs. (b) we present the design and implementation of \name to overcome these inefficiencies, (c) through testbed prototype and simulation, we show that \name balances the traffic as per capacities and improves latency by up to 80\%.  
\fi 

\if 0
\name is based on 4 key ideas. First, it uses end-to-end latency and packet drop between the requests and responses as a capacity congestion signal. We observe that when traffic reaches the capacity for most of the components (CPU, network etc.), it results in increased end-to-end latency and packet drops due to queuing delays as well as contention. Thus, by monitoring the latency and drop, we gauge if traffic is reaching the capacity of the DIPs. 

Second, we formulate an Integer Linear Program (ILP) to calculate the LB weights to minimize the total latency while ensuring there are no packet drops. As detailed in \S\ref{}, the ILP takes the mapping between weights and latency as an input. However, building such a mapping at scale with 100s of points for each DIP is challenging. Additionally, again at scale, the ILP also becomes computationally expensive and takes long time to run.

Our third key idea is to speed up building the mapping between weights and latency for individual DIPs. We observed that we don't need to calculate latency at different weights for all DIPs. Instead we can measure latency at a few weights and use curve fitting. We use a novel idea inspired by TCP congestion control to hop different weights and measure latency. Additionally, we use a novel idea of \textit{scheduling measurements} to prioritize certain latency measurements over others. Lastly, we use clustering using K-means to club DIPs with similar characteristics. 

We implemented \name of a testbed with 40 DIPs and 
\fi


==> old-intro.tex <==
\section{Introduction}
\label{sec:intro}

A high performance layer-4 load balancer (L4 LB) is one of the key building blocks of online services. Individual services running inside clusters expose a small number of virtual IPs, termed {\em VIPs}, to receive external Internet traffic. Internally, services run on multiple backend servers or VMs with unique IP addresses. Henceforth, we will refer to backend instances as {\em DIPs}. The LB receives traffic coming on the VIPs and distributes it across DIPs. Recently, a significant number of efforts have focused on improving the scale, availability and cost of the LB~\cite{ananta:sigcomm13, maglev:nsdi16, duet:sigcomm14, silkroad:sigcomm17, beamer:nsdi18, cheetah:nsdi20, tiara:nsdi22}. 

%% Previous work on load balancing assume that capacity of the DIPs is uniform and/or static (\S\ref{sec:related}). 
%% such works have fallen short regarding the fundamental goal of load-balancer, \ie to load-balance the traffic as per the capacities of the DIPs. 
%% However, 
There is a growing trend that DIPs exhibit different and time-varying capacities, especially in virtualized clusters. Prior work has shown that the request-processing rates of VMs with the same type (\eg D3.medium) may vary up to 40\% due to \textit{noisy neighbors} (\S\ref{sec:related}). VMs on the same host compete for shared resources such as caches and memory buses, resulting in variation. Additionally, DIPs in the same DIP-pool may be provisioned with different capacities (\S\ref{sec:back}). Recent proposals and new offerings from cloud providers introduce dynamic changes to the number of virtual CPUs assigned to VMs (\S\ref{sec:back})\ngs{$\leftarrow$ citation required}. Together, these factors result in different (and dynamic) capacities across DIPs and over time.

We measure the impact of having DIPs with different capacities on load balancing -- specifically, whether the LB splits the traffic as per capacities of DIPs. We evaluate using: (a) HAProxy LB -- one of the widely used open source LB with all available algorithms, (b) Azure LB. We observed that the algorithms fell short in splitting traffic as per the capacities – overutilizing some DIPs while underutilizing the rest. Interestingly, least connection based algorithm that is specifically built to adapt to different capacities fell short. As a result, the requests going to the over-utilized DIPs observed 2$\times$ higher latency than other DIPs. Lastly, existing LB designs remove the DIP suffering from poor performance – instead of adapting to its capacity.
\ngs{reminder: these experiments show we are better than existing ``practical'' load balancers, but we should make a comparison/show an improvement relative to more `academic' load balancers from the literature. It is definitely doable.}

In this paper, we revisit the first order question on how L4 LBs split traffic. We argue that, going forward, there is a need for \textit{load bin-packing} -- systems that pack the load as per capacities of the DIPs. To that extend, we present \name. The goal of \name is not to add to the impressive list of existing LB designs. Instead, it compliments the existing designs by specifying the weights for splitting the traffic across DIPs. \name frees up admins from deciding weights when capacities are static or dynamic. In doing so, it combines the best of both worlds -- it compliments the availability, scalability and cost benefits of the existing LB designs with weight calculations as per the capacities. A significant number of LB systems provide an interface to specify the weights including AVI\cite{avi:web}, Nginx\cite{nginx:web}, Duet\cite{duet:sigcomm14}, HAProxy\cite{haproxy:web}. \name continually evaluates the capacities of DIPs and sets the weights accordingly. This way \name empowers other LBs to be capacity-aware.

\name is based on three key ideas. First, inspired by SDN principles, it decouples the weight calculation from individual LB instances, and calculates the weights at a central controller. The benefits are twofold: (a) it frees up LB dataplane from weight calculation and helps it to be high performant and provide low latency, high throughput packet processing, (b) it helps implement more informed designs for weight calculation at the central controller. 

%% \name uses an ILP (detailed below) at the controller to calculate weights using end-to-end latency between requests and responses.

%% We observe that when traffic reaches the capacity of the DIPs, it results in increased end-to-end latency and packet drops due to queuing delays and contention. Thus, by monitoring the latency and drop, we gauge if traffic is reaching the capacity of the DIPs. 

Second, as a part of load packing, we formulate an Integer Linear Program (ILP) to calculate the LB weights to minimize the total end-to-end latency across DIPs of a VIP as applications value better latencies. While an ILP based packing is appealing, it is also challenging. As detailed in \S\ref{sec:ilp}, the ILP takes the mapping between weights and latency as an input. However, building such a mapping at scale with 100s of latency measurements for each DIP is not trivial. Additionally, again at scale, the ILP becomes computationally expensive.

Our third key idea is to speed up building the mapping between weights and latency for individual DIPs. We observed that we can make-do with latency measurement at small number of weights and use curve-fitting. Next, we use an idea inspired by TCP congestion control to hop different weights to reduce number of latency measurements and get rough estimate of capacity of DIPs. Lastly, we use multi-step ILP to substantially speed up weight calculation. 

To the best of our knowledge, \name is a novel approach to build capacity aware L4 LBs. We evaluate \name using prototype implementation and simulations. Our results show: (1) \name can adjust the weights as per the capacities of the DIPs. (2) In doing so, it cuts the latency up to 45\% for up to 79\% requests. (3) \name adapts to dynamics in the cluster such as capacity, traffic changes and DIP failures. (4) \name is fast using different optimizations and solves the ILP quickly. (5) \name incurs only a small overhead in terms of \#cores and costs.

This work does not raise any ethical issues.

\if 0
In summary, we make the following contributions: (a) we show that existing LB algorithms (especially least connection algorithm tailored for handling different capacities) fall short in load balancing traffic as per capacities of the DIPs. (b) we present the design and implementation of \name to overcome these inefficiencies, (c) through testbed prototype and simulation, we show that \name balances the traffic as per capacities and improves latency by up to 80\%.  
\fi 

\if 0
\name is based on 4 key ideas. First, it uses end-to-end latency and packet drop between the requests and responses as a capacity congestion signal. We observe that when traffic reaches the capacity for most of the components (CPU, network etc.), it results in increased end-to-end latency and packet drops due to queuing delays as well as contention. Thus, by monitoring the latency and drop, we gauge if traffic is reaching the capacity of the DIPs. 

Second, we formulate an Integer Linear Program (ILP) to calculate the LB weights to minimize the total latency while ensuring there are no packet drops. As detailed in \S\ref{}, the ILP takes the mapping between weights and latency as an input. However, building such a mapping at scale with 100s of points for each DIP is challenging. Additionally, again at scale, the ILP also becomes computationally expensive and takes long time to run.

Our third key idea is to speed up building the mapping between weights and latency for individual DIPs. We observed that we don't need to calculate latency at different weights for all DIPs. Instead we can measure latency at a few weights and use curve fitting. We use a novel idea inspired by TCP congestion control to hop different weights and measure latency. Additionally, we use a novel idea of \textit{scheduling measurements} to prioritize certain latency measurements over others. Lastly, we use clustering using K-means to club DIPs with similar characteristics. 

We implemented \name of a testbed with 40 DIPs and 
\fi


==> overview-back.tex <==
\section{\name}
\label{sec:overview}

\subsection{Goals}

We present \name, a ``meta'' (to handle weights) LB designed to meet the following
goals:

\textbf{Generality}: \name intends to work with existing LB
designs without any changes to MUXes, DIPs or
clients. It seeks to free up existing LB/MUXes from all capacity related
calculations.

\textbf{Performance-aware LB}: 
Our vision is that users can plugin any DIP, and \name should balance load to optimize for service response latency
\textit{without taking any input hints} about the
capacities or performance. Additionally, \name should adjust load when the performance changes dynamically. In essence, \name must free-up admins from the
labor of setting up configurations for performance-aware LBs.

%% \name should do capacity aware load balancing not only when capacities change dynamically but also when DIPs have statically different capacities (e.g., DIPs with 1 and 4 cores). \name should not require any \textit{hints} about capacities.

%%\textbf{Load balance across DIPs of any capacity!}: Goal of \name is to load balance traffic across DIPs of heterogeneous and dynamic capacities without any restrictions on the number and capacities of DIPs. \name should not require any \textit{hints} about the capacities.

%% \name should work even when capacities of DIPs are vastly different.

%%  Similarly, \name should not run any agents on the
%% MUXes, DIPs or clients.

\textbf{Zero-touch and agent-less design:} \name should work with
unmodified DIPs, MUXes and clients -- it does not have access to
these components.  
\name should work without access to DIP SKU, CPU utilization, or any
performance counters on DIPs. This goal helps customers maintain privacy about their resource usage, and helps \name reduce deployment overheads.

\textbf{Everything online}: \name should not require any offline
profiling data. Using just the IP addresses of the DIPs, \name should
perform its functions online.

%% Application Latency as a Performance Signal

\subsection{Load balancing by controlling weights to optimize for application latency}
\label{sec:overview:latency}

\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth, page=3]{figs/design-cpu-latency.pdf}
\caption{Impact of increasing weights (traffic) on latency (y2 axis) and CPU utilization (y1 axis). TCP and ICMP pings are unaffected by changing weights (traffic).}
\label{fig:design:weight}
\end{figure}


%%As shown in Fig.\ref{fig:back:burst}, the latency varies 10$\times$ for the same CPU utilization measured within VM.

\name casts the LB problem as a Knapsack problem to pack the load according to the capacities of the DIPs to improve the application latency. As mentioned above \name intends to work with existing LB designs without agents on MUXes, DIPs or clients. 

\textbf{Using weights to adjust traffic:} We use \textit{weights} as levers  to adjust the traffic. That's because: (a) we observe that many existing LB designs provide an interface to specify the weights for splitting the traffic. \name uses this interface to program the weights. This way, \name can support a
variety of other LBs. Wherever such an interface is not provided, we
use DNS based load balancing (an example in
\S\ref{sec:eval:other}). Importantly, the MUXes themselves remain unmodified and
their throughput and latency are unaffected by \name. (b) \name does not have dataplane details such as amount of traffic going to each DIP. Note that LB dataplane implementations are specific to individual LBs such as Ananta that uses IP-in-IP, or HAProxy that uses separate connections. Additionally, the dataplane is controlled by LB control plane that is not publicly available. As a results \name does not have visibility into the amount of traffic going into each DIP or the total traffic. As we show in \S\ref{sec:testbed}, \name works well even when simply using weights.

\textbf{Using application latency as a feedback:} \name monitors the \textit{service (application) latency} to individual DIPs and uses it to pack the load so as to minimize total latency across DIPs (more details in \S\ref{sec:ilp}). To do so, it sends application requests (such as HTTP) to the DIPs and measures the request-response latency for such requests. The reasons are following: (a) alternatives could be to simply use monitor load through CPU utilization on DIPs. However, it will either require agents on the DIPs or access to client subscription -- both raising privacy concerns and are non-goals for \name. (b) Service latency is not a function of just CPU utilization.  Application latency also depends on many factors across the stack such as CPU cache at hardware\cite{slomo:sigcomm20}, throttling at hypervisor as well as application related factors (such as queues). It is not trivial to capture and translate multitude resource counters to application performance\cite{slomo:sigcomm20}. (c) Application latency closely captures the service performance, and eliminates the need to capture and translate multitude signals from hardware to software. 

Lastly, \name uses application latency instead of ICMP ping or TCP ping (using SYN/SYN-ACK) as they do not reflect the load on the DIP. Fig.\ref{fig:design:weight} shows the change in appliction (app), and ICMP and TCP pings as we vary the weights/traffic. ICMP and TCP pings are handled by OS, whereas the application pings are handled by application and reflect the performance of the applications. 

\subsection{\name Overview and Architecture}
\label{sec:overview:overv}

\name is generic and can be deployed in any cloud or enterprise. 
%% It does not require any admin data/access and completely runs in user space.
%%incorporates a feedback control loop designed to make existing LBs capacity aware, with weights reflecting the  capacities of DIPs.
%
\name has three key aspects: (a)
gauging \textit{DIP performance vs. weights}, through an active
probing approach (\S\ref{sec:design:curve}, \S\ref{sec:design:measure}) that works out-of-band, without DIP, MUX,
or client modification, (b) weight computation at a centralized
controller, that uses a multi-step ILP (\S\ref{sec:design:runtime}) with the goal of
packing load into DIPs to minimize average response latency, and
(c) programming the DIP weights on the fast data path.
%


%% \subsection{Architecture}
\label{sec:overview:arch}

%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth]{figs/design-block.pdf}
\caption{\name architecture. Blue boxes denote \name components. Solid and dotted lines denote data traffic and control signals respectively.}
\label{fig:overview:arch}
\vspace{-0.15in}
\end{figure}
%%%%%% end figure %%%%%%%%%%%%%%%%%

\begin{table}[t]
\centering
\caption{Notations used in the ILP.}
\label{tab:algo:notation}
{
\small
\begin{tabular} {|c|c|}
\hline
\textbf{Notation} & \textbf{Explanation}\\
\hline
\hline
\multicolumn{2}{|c|}{Input} \\
\hline
$D$ & Set of DIPs \\
\hline
$w$ & Weight between [0,1]\\
\hline
$W_{d}$ & Set of weights for d-th DIP\\
\hline
$l_{d,w}$ & Latency on d-th DIP for w-th weight\\
\hline
$y_{max},$  & Max. and min. weights \\
$y_{min}$ & across DIPs\\
\hline
\hline 
%% \multicolumn{2}{|c|}{Output Variable (binary)} \\
%%\hline
(output) & Set if w-th weight is assigned \\
$X_{d,w}$ &  to d-th DIP\\
\hline
\end{tabular}
}
\end{table}

\if 0
%%%%%% begin figure %%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth]{figs/design-ping-latency.pdf}
\caption{End-to-end (round-trip) latency using different mechanisms.}
\label{fig:overview:latency}
\end{figure}
%%%%%% end figure %%%%%%%%%%%%%%%%%
\fi

%% As we detail in the next section, the controller calculates the weights using Integer Linear Program (ILP) to minimize the total latency across all DIPs of a VIP (we run ILP separately for individual VIPs). 

%% To do so, inspired by SDN principles, \name chooses to decouple the weight calculation from existing LB designs (especially from MUXes) and calculates weights  at a central controller.  It paves way to make decisions optimally while MUXes focus on packet processing with low latency and high throughput. 

As shown in  Fig.\ref{fig:overview:arch}, \name consists of three
loosely coupled components: (a) KLM (\name Latency Measurement), (b)
latency store, and (c) controller.

KLM resides in each customer-level virtual network (VNET). For
simplicity, we assume there is one externally-visible VIP per
VNET. KLM periodically measures the latency for requests from each
DIP.  KLM directly
measures the latency at the application-level (\eg HTTP requests)
using service URLs provided by the administrators.  KLM also
sends requests directly to the DIPs (using IPs of DIPs; bypassing MUXes) to eliminate
the interference of the MUXes on DIP latency. The latency store persists the measurements from the KLM. Implementing
measurements out-of-band (with respect to
the critical request-processing path) and storing them separately
enables \name to avoid changes to the MUXes, servers and clients,
broadening \name's utility to a variety of LBs and settings.

%% NGS: seems very implementation specific
%% We provide a VM image to
%% run KLM. Admins simply need to run the KLM in their VNET (more
%% details in \S\ref{sec:impl}) and add the DIPs and URL to a config
%% file.

The \name controller consumes DIP latencies from the latency store. It
computes the weights using Integer Linear Program (\S\ref{sec:ilp}) and sends
them to the LB controller (e.g., Ananta, HAProxy), which in turn
programs the MUXes with the new weights. The MUXes may implement the
weights using WRR (weighted round robin). Existing LB controllers are
\textit{not} on the critical path of the traffic\cite{ananta:sigcomm13,
  maglev:nsdi16}. Likewise, \name controller is not on the
critical path. Lastly, the \name controller also includes techniques
to handle failures and traffic changes (\S\ref{sec:dynamics}).


==> schedule-old.tex <==
\subsection{Scheduling Measurements}
\label{sec:design:schedule}
In \name, the weights for those DIPs with $isExplorationDone$ set are
calculated by ILP, and we use the algorithm from
\S\ref{sec:design:measure} to calculate the weights for the remaining
DIPs. For such DIPs, however, we may not be able to measure latency
for the calculated weights right away, as the sum of all DIP weights
for a VIP needs to be 1. The sum of weights calculated
in \S\ref{sec:design:measure} may not always be 1, \eg $w_{next}$ for
2 DIPs can be 0.7 each in one iteration. In such scenarios, we need to
\textit{schedule} the DIP weight in multiple rounds, and we
need to determine weights to schedule in each round.

To prioritize our measurements, we classify DIPs with new weights
(with $isExplorationDone$ unset) to be scheduled into 3 priority
classes: (a) weights for over-utilized DIPs (DIPs with large latency), \ngs{how do you identify
  this?} (b) weights for remaining DIPs, (c) weights during
refresh. Within a class, we use FIFO. To schedule the DIPs that have
new weights assigned, we use a simple greedy algorithm where we
arrange all DIPs according to their priority. We hop over the list of
DIPs until either (1) the weight of DIPs scheduled is 1, or (2) we
have exhausted the list of DIPs.

It can happen that the total weight for the scheduled DIPs is less
than 1 (especially in case (2) above). If this occurs, we calculate
the remaining weights for DIPs as follows. Suppose the total weight
assigned by the scheduler is $w_{s}$. Hence, we need to assign $1 -
w_{s}$ using the remaining DIPs. For the DIPs where we have
$isExplorationDone$ flag set, we use the ILP with a modified
constraint (b) in Fig.\ref{fig:algo:lp} where the total weight is $1 -
w_{s}$. In cases where the ILP returns \textit{unsatisfiable} with
this constraint, we split the remaining weight (1 -- $w_{s}$) equally
across all remaining DIPs.
